Breaking bad theories of class $\mathcal S$

We study weakly-coupled descriptions/channel decompositions of the 4d $\mathcal{N}=2$ theories of class $\mathcal{S}$ of type $\mathfrak{su}(N)$, from the perspective of the 3d $\mathcal{N}=4$ mirror duals of their circle compactifications. This is a delicate problem when the channel decomposition produces pathological, or bad, 4d configurations that correspond to spheres with non-maximal punctures. The star-shaped quivers, describing the 3d mirrors associated with such bad 4d configurations, are bad 3d $\mathcal{N}=4$ theories. Leveraging recent results regarding 3d bad theories, we identify a new and interesting family of bad theories, which we coin \textit{broken} theories, that naturally arise in this context. Using these broken theories, we develop a systematic and analytic method that determines the generically non-Lagrangian matter sectors and the weakly-coupled gauge groups in such channel decompositions. We understand these weakly-coupled descriptions as emerging dynamically via Higgs mechanisms triggered by operators acquiring vacuum expectation values.

==> custom_commands.tex <==

% ======================================================
%   COLORS
\definecolor{CScolor}{rgb}{1.0, 0.0, 0.0}
\colorlet{BFcolor}{OliveGreen}
\colorlet{FIcolor}{orange}

% \definecolor{BFcolor} {RGB} {0, 158, 96} % BF
% \definecolor{FIcolor}{RGB}{250, 95, 85} % FI
% \definecolor{CScolor}{RGB}{255, 36, 0} % CS


% ======================================================
%   SYMBOLS SHORTCUTS
\def\mon{\mathfrak{M}}

\def\identityN[#1,#2]{
	_{#1}\mathbb{I}_{#2}^{[N]}
}

\def\identityOne[#1,#2]{
	_{#1}\mathbb{I}_{#2}^{[1^N]}
}

\def\DeltaN[#1]{
	\Delta^{[N]}\left( #1 \right)
}

\def\DeltaOne[#1]{
	\Delta^{[1^N]}\left( #1 \right)
}


%========================================================
% Mathematical Symbols 
\def\half{\frac{1}{2}}
\def\imp{\Longrightarrow}
\def\goto{\rightarrow}
\def\para{\parallel}
\def\vev#1{\langle #1 \rangle}
\def\del{\nabla}
\def\p{\partial}
\newcommand{\bra}[1]{\langle{#1}|}
\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\lra}{\leftrightarrow}


% ======================================================
% TEX ENVIRONMENTS
\newenvironment{proposal}[1][Proposal]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}



%=====================================================
% arrows and styles for flavor and gauge nodes
\tikzstyle{flavor}=[rectangle,draw=black,thick,inner sep = 0pt, minimum size = 6mm]
\tikzstyle{manifest}=[rectangle,draw=blue!50,thick,inner sep = 0pt, minimum size = 6mm]
\tikzstyle{gauge2}=[circle,draw=black,thick,inner sep = 0pt, minimum size = 6mm] %regular gauge node
\tikzstyle{gauge}=[rounded rectangle,draw=black,thick,inner sep = 0pt, minimum size = 6mm] % node for long labels
% Palash: I have swapped gauge and gauge2 from "default"

\tikzset{->-/.style={decoration={
  markings,
  mark=at position .5 with {\arrow{>}}},postaction={decorate}}}
\tikzset{-<-/.style={decoration={
  markings,
  mark=at position .5 with {\arrow{<}}},postaction={decorate}}}
\tikzstyle{BFline}=[dashed]

\tikzstyle{hyper}=[-,thick]
\tikzstyle{FI}=[FIcolor,font=\small]
  
% ======================================================
% QUIVER NODES AND ARROWS
\def\nodeCS(#1,#2)(#3,#4,#5){ 	% nodeCS(x,y)(nodename,nodelabel, CSlevel)
	\node at (#1,#2) (#3) [gauge,black] {#4};
	\draw[CScolor] (#3) ++(6pt,-7pt) node[anchor=west] {\tiny#5};
}

\def\flavorCS(#1,#2)(#3,#4,#5){ 	% nodeCS(x,y)(nodename,nodelabel, CSlevel)
	\node at (#1,#2) (#3) [flavor,black] {#4};
	\draw[CScolor] (#3) ++(6pt,-8pt) node[anchor=west] {\tiny#5};
}

\def\arrowBF(#1,#2)(#3){ %\arrowBF(node1, node2) (BFlevel)
	\begin{scope}[every node/.style={auto, outer sep=-1pt}]
	\path (#1) edge[->-] node[BFcolor,midway] {\tiny#3} (#2);
	\end{scope}
}

\def\arrowBFlr(#1,#2)(#3,#4){ %\arrowBF(node1, node2) (BFlevel, left/right)
	\begin{scope}[every node/.style={auto=#4, outer sep=-1pt}]
	\path (#1) edge[->-] node[BFcolor,midway] {\tiny#3} (#2);
	\end{scope}
}

\def\dottedBF(#1,#2)(#3){ %\arrowBF(node1, node2) (BFlevel)
	\begin{scope}[every node/.style={auto, outer sep=-1pt}]
	\path (#1) edge[dashed] node[BFcolor,midway] {\tiny#3} (#2);
	\end{scope}
}


%=====================================================
% COMPACT FUNDAMENTAL BLOCKS
\def\simpFund[#1]{ % #1 is N
	\begin{tikzpicture}
        \node at (0,0) (g) [flavor, black] {$#1$};
        \node at (0,1.5) (f) [flavor,black] {$1$};
        \draw[CScolor] (g)+(0,-.6) node {$_{( \text{-}\frac{1}{2}, \text{-}\frac{1}{2})}$};
        %\draw[CScolor,right] (f2)+(.2,-.4) node {$_{\text{-}\frac{#1}{2}}$};
        %\draw[BFcolor,left] (-.1,.75) node {$_{+1}$};
        \draw[->-] (g)--(f);
        \draw[right] (g)+(.4,0) node {$\mathbb{I}^{[#1]}$};
	\end{tikzpicture}
}

\def\simpAFund[#1]{ % #1 is N
	\begin{tikzpicture}
        \node at (0,0) (g) [flavor, black] {$#1$};
        \node at (0,1.5) (f) [flavor,black] {$1$};
        \draw[CScolor] (g)+(0,-.6) node {$_{(\text{-}\frac{1}{2}, \text{-}\frac{1}{2})}$};
        %\draw[CScolor,right] (f2)+(.2,-.4) node {$_{\text{-}\frac{#1}{2}}$};
        %\draw[BFcolor,left] (-.1,.75) node {$_{+1}$};
        \draw[->-] (f)--(g);
        \draw[right] (g)+(.4,0) node {$\mathbb{I}^{[#1]}$};
	\end{tikzpicture}
}

\def\simpFundNMirror[#1]{ % #1 is N
	\begin{tikzpicture}
		\node at (-1.5,0) (f1) [flavor,black] {$#1$};
        \node at (0,0) (g1) [gauge, black] {$1^#1$};
        \node at (1,1) (g2) [gauge,black] {$1^#1$};
        \node at (2.5,1) (f2) [flavor,black] {$#1$};
        \draw[->-] (g1)--(g2);
        \draw[decorate,decoration={coil,segment length=4pt}] (f1)--(g1) node[midway,above] {$+$};
        \draw[decorate,decoration={coil,segment length=4pt}] (g2)--(f2)node[midway,above] {$-$};
	\end{tikzpicture}
}

\def\simpAFundNMirror[#1]{
	\begin{tikzpicture}
		\node at (-1.5,1) (f1) [flavor,black] {$#1$};
        \node at (0,1) (g1) [gauge, black] {$1^#1$};
        \node at (1,0) (g2) [gauge,black] {$1^#1$};
        \node at (2.5,0) (f2) [flavor,black] {$#1$};
        \draw[->-] (g2)--(g1);
        \draw[decorate,decoration={coil,segment length=4pt}] (f1)--(g1) node[midway,above] {$+$};
        \draw[decorate,decoration={coil,segment length=4pt}] (g2)--(f2)node[midway,above] {$-$};
	\end{tikzpicture}
}

\def\simpBifLNN[#1]{
	\begin{tikzpicture}
        \node at (0,0) (g) [flavor, black] {$#1$};
        \node at (1.5,0) (f) [flavor,black] {$#1$};
        \draw[CScolor] (g)+(0,-.6) node {$_{(\text{-}\frac{#1}{2},\text{-}\frac{#1}{2})}$};
        \draw[CScolor] (f)+(0,-.6) node {$_{(\text{-}\frac{#1}{2},\text{-}\frac{#1}{2})}$};
        \draw[BFcolor] (.75,.3) node {$_{+1}$};
        \draw[->-] (f)--(g);
	\end{tikzpicture}
}

\def\simpBifRNN[#1]{
	\begin{tikzpicture}
		\node at (0,0) (g) [flavor, black] {$#1$};
        \node at (1.5,0) (f) [flavor,black] {$#1$};
        \draw[CScolor] (g)+(0,-.6) node {$_{(\text{-}\frac{#1}{2},\text{-}\frac{#1}{2})}$};
        \draw[CScolor] (f)+(0,-.6) node {$_{(\text{-}\frac{#1}{2},\text{-}\frac{#1}{2})}$};
        \draw[BFcolor] (.75,.3) node {$_{+1}$};
		\draw[->-] (g)--(f);
	\end{tikzpicture}
}

\def\simpBifLNNMirror[#1]{
\;
	\begin{tikzpicture}
		\node at (-1.5,0) (f1) [flavor,black] {$#1$};
        \node at (0,0) (g) [gauge, black] {$1^#1$};
        \node at (1.5,0) (f2) [flavor,black] {$#1$};
        \node at (1,-1) (f3) [flavor,black] {$1$};
        \draw[decorate,decoration={coil,segment length=4pt}] (f1)--(g) node[midway,above] {$+$};
        \draw[decorate,decoration={coil,segment length=4pt}] (g)--(f2)node[midway,above] {$-$};
		\draw[->-] (f3)--(g);
	\end{tikzpicture}
\;
}

\def\simpBifRNNMirror[#1]{
\;
	\begin{tikzpicture}
		\node at (-1.5,0) (f1) [flavor,black] {$#1$};
        \node at (0,0) (g) [gauge, black] {$1^#1$};
        \node at (1.5,0) (f2) [flavor,black] {$#1$};
        \node at (-1,1) (f3) [flavor,black] {$1$};
        \draw[decorate,decoration={coil,segment length=4pt}] (f1)--(g) node[midway,above] {$+$};
        \draw[decorate,decoration={coil,segment length=4pt}] (g)--(f2)node[midway,above] {$-$};
		\draw[->-] (g)--(f3);
	\end{tikzpicture}
\;
}

\def\simpGenBifund[#1]{ % #1 is N
\;
	\begin{tikzpicture}[baseline=0]
		    \node at (0,0) (g1) [flavor, black] {$#1$};
		    \node at (1.3,0) (f1) [flavor,black] {$1^#1$};
		    \draw[decorate,decoration={coil,segment length=4pt}] (f1)--(g1);
	\end{tikzpicture}
}

\def\simpGenBifundA[#1]{ % #1 is N
\;
	\begin{tikzpicture}[baseline=0]
		    \node at (0,0) (g1) [flavor, black] {$1^#1$};
		    \node at (1.3,0) (f1) [flavor,black] {$#1$};
		    \draw[decorate,decoration={coil,segment length=4pt}] (f1)--(g1);
	\end{tikzpicture}
}

\def\simpBifLOne[#1]{
\;
	\begin{tikzpicture}[baseline=10]
		    \node at (1,0) (g) [flavor, black] {$#1$};
		    \node at (0,1) (f) [flavor,black] {$#1$};
		    \draw[->-] (g)--(f);
	\end{tikzpicture}
\;
}

\def\simpBifROne[#1]{
\;
	\begin{tikzpicture}[baseline=10]
		    \node at (0,0) (g) [flavor, black] {$#1$};
		    \node at (1,1) (f) [flavor,black] {$#1$};
		    \draw[->-] (g)--(f);
	\end{tikzpicture}
\;
}

\def\simpFundOneMirror[#1]{
\;
	\begin{tikzpicture}[baseline=0]
		\node at (-1.5,0) (f1) [flavor,black] {$1^#1$};
		    \node at (0,0) (g1) [gauge, black] {$#1$};
      \draw[red] (-.5,-.6) node {$_{(-\frac{1}{2}, #1-\frac{1}{2})}$};
        \draw[OliveGreen] (.5,.5) node {$_1$};
      \draw[red] (1.5,-.6) node {$_{(-\frac{1}{2}, #1-\frac{1}{2})}$};
		    \node at (1,0) (g2) [gauge,black] {$#1$};
		    \node at (2.5,0) (f2) [flavor,black] {$1^#1$};
		    \draw[->-] (g1)--(g2);
		    \draw[decorate,decoration={coil,segment length=4pt}] (f1)--(g1) node[midway,above] {$+$};
			\draw[decorate,decoration={coil,segment length=4pt}] (g2)--(f2)node[midway,above] {$-$};
	\end{tikzpicture}
\;
}

\def\simpFundOne[#1]{
\;
	\begin{tikzpicture}[baseline=0]
		    \node at (0,0) (g1) [flavor, black] {$1^#1$};
		    \node at (0,1.5) (f2) [flavor,black] {$1$};
		    \draw[->-] (g1)--(f2);
	\end{tikzpicture}
\;
\mathbb{I}^{[1^#1]}
\;
}

\def\simpAFundOneMirror[#1]{
\;
	\begin{tikzpicture}[baseline=0]
		\node at (-1.5,0) (f1) [flavor,black] {$1^#1$};
		    \node at (0,0) (g1) [gauge, black] {$#1$};
      \draw[red] (-.5,-.6) node {$_{(-\frac{1}{2}, #1-\frac{1}{2})}$};
        \draw[OliveGreen] (.5,.5) node {$_1$};
      \draw[red] (1.5,-.6) node {$_{(-\frac{1}{2}, #1-\frac{1}{2})}$};
		    \node at (1,0) (g2) [gauge,black] {$#1$};
		    \node at (2.5,0) (f2) [flavor,black] {$1^#1$};
		    \draw[->-] (g2)--(g1);
		    \draw[decorate,decoration={coil,segment length=4pt}] (f1)--(g1) node[midway,above] {$+$};
			\draw[decorate,decoration={coil,segment length=4pt}] (g2)--(f2)node[midway,above] {$-$};
	\end{tikzpicture}
\;
}

\def\simpAFundOne[#1]{
\;
	\begin{tikzpicture}[baseline=0]
		    \node at (0,0) (g1) [flavor, black] {$1^#1$};
		    \node at (0,-1.5) (f2) [flavor,black] {$1$};
		    \draw[->-] (f2)--(g1);
	\end{tikzpicture}
\;
\mathbb{I}^{[1^#1]}
\;
}

\def\simpBifLOneMirror[#1]{
\;
	\begin{tikzpicture}[baseline=0]
		\node at (-1.5,0) (f1) [flavor,black] {$1^#1$};
		    \node at (0,0) (g) [gauge, black] {$#1$};
                \draw[red] (0,-.6) node {$_{(-\frac{1}{2}, #1-\frac{1}{2})}$};
		    \node at (1.5,0) (f2) [flavor,black] {$1^#1$};
		 	 \node at (-1.5,1) (f3) [flavor,black] {$1$};
		    \draw[decorate,decoration={coil,segment length=4pt}] (f1)--(g) node[midway,above] {$+$};
			\draw[decorate,decoration={coil,segment length=4pt}] (g)--(f2)node[midway,above] {$-$};
		\draw[->-] (f3)--(g);
	\end{tikzpicture}
\;
}

\def\simpBifROneMirror[#1]{
\;
	\begin{tikzpicture}[baseline=0]
		\node at (-1.5,0) (f1) [flavor,black] {$1^#1$};
		    \node at (0,0) (g) [gauge, black] {$#1$};
         \draw[red] (-.5,-.6) node {$_{(-\frac{1}{2}, #1-\frac{1}{2})}$};
		    \node at (1.5,0) (f2) [flavor,black] {$1^#1$};
		 	 \node at (1.5,-1) (f3) [flavor,black] {$1$};
		    \draw[decorate,decoration={coil,segment length=4pt}] (f1)--(g) node[midway,above] {$+$};
			\draw[decorate,decoration={coil,segment length=4pt}] (g)--(f2)node[midway,above] {$-$};
		\draw[->-] (g)--(f3);
	\end{tikzpicture}
\;
}


%=====================================================
% TIKZ STYLES
\tikzset{cross/.style={cross out, draw=black, minimum size=5*(#1-\pgflinewidth), inner sep=0pt, outer sep=0pt},
%default radius will be 1pt. 
cross/.default={2pt}}

\tikzset{snake it/.style={decorate, decoration=snake}}

\tikzset{mid arrow/.style={postaction={decorate,decoration={
        markings,
        mark = at position .55 with {\arrow[#1]{Straight Barb[width=5pt]}}
      }}}}
      
\tikzset{mid arrowsm/.style={postaction={decorate,decoration={
        markings,
        mark = at position .55 with {\arrow[#1]{Straight Barb[width=3pt]}}
      }}}}
      
\tikzset{middx arrowsm/.style={postaction={decorate,decoration={
        markings,
        mark = at position .7 with {\arrow[#1]{Straight Barb[width=3pt]}}
      }}}}
      
\tikzset{midsx arrowsm/.style={postaction={decorate,decoration={
        markings,
        mark = at position .4 with {\arrow[#1]{Straight Barb[width=3pt]}}
      }}}}




  
\newcommand{\wigE}{\draw[snake=zigzag]}
\newcommand{\orwigE}{\draw[snake=zigzag,orange]}
%\newcommand{\wigM}{\draw[snake=coil,segment length=3pt]}
\newcommand{\wigM}{\draw[snake=coil,,segment aspect=0,segment length=6pt, double]}
\newcommand{\wigMc}{\draw[->,snake=coil,segment aspect=0,segment length=6pt]}
\newcommand{\wigMB}{\draw[->,snake=zigzag,segment aspect=0,segment length=6pt]}
\newcommand{\wigT}{\draw[dashed]}
\newcommand{\NSbrane}{\draw[ultra thick, blue]}
\newcommand{\Dbrane}{\draw[dashed, ultra thick, gray]}
\newcommand{\Dthree}{\draw[thick, red]}
\newcommand{\hyper}{\draw[-,double distance=3]}
\newcommand{\chir}{\draw[-,mid arrow]}

\newcommand{\convexpath}[2]{
[   
    create hullnodes/.code={
        \global\edef\namelist{#1}
        \foreach [count=\counter] \nodename in \namelist {
            \global\edef\numberofnodes{\counter}
            \node at (\nodename) [draw=none,name=hullnode\counter] {};
        }
        \node at (hullnode\numberofnodes) [name=hullnode0,draw=none] {};
        \pgfmathtruncatemacro\lastnumber{\numberofnodes+1}
        \node at (hullnode1) [name=hullnode\lastnumber,draw=none] {};
    },
    create hullnodes
]
($(hullnode1)!#2!-90:(hullnode0)$)
\foreach [
    evaluate=\currentnode as \previousnode using \currentnode-1,
    evaluate=\currentnode as \nextnode using \currentnode+1
    ] \currentnode in {1,...,\numberofnodes} {
  let
    \p1 = ($(hullnode\currentnode)!#2!-90:(hullnode\previousnode)$),
    \p2 = ($(hullnode\currentnode)!#2!90:(hullnode\nextnode)$),
    \p3 = ($(\p1) - (hullnode\currentnode)$),
    \n1 = {atan2(\y3,\x3)},
    \p4 = ($(\p2) - (hullnode\currentnode)$),
    \n2 = {atan2(\y4,\x4)},
    \n{delta} = {-Mod(\n1-\n2,360)}
  in 
    {-- (\p1) arc[start angle=\n1, delta angle=\n{delta}, radius=#2] -- (\p2)}
}
-- cycle
}


